Performance Portable Back-projection Algorithms on CPUs: Agnostic Data Locality and Vectorization Optimizations

Computed Tomography (CT) is a key 3D imaging technology that fundamentally relies on the compute-intense back-projection operation to generate 3D volumes. GPUs are typically used for back-projection in production CT devices. However, with the rise of power-constrained micro-CT devices, and also the emergence of CPUs comparable in performance to GPUs, back-projection for CPUs could become favorable. Unlike GPUs, extracting parallelism for back-projection algorithms on CPUs is complex given that parallelism and locality are not explicitly defined and controlled by the programmer, as is the case when using CUDA for instance. We propose a collection of novel back-projection algorithms that reduce the arithmetic computation, robustly enable vectorization, enforce a regular memory access pattern, and maximize the data locality. We also implement the novel algorithms as efficient back-projection kernels that are performance portable over a wide range of CPUs. Performance evaluation using a variety of CPUs from different vendors and generations demonstrates that our back-projection implementation achieves on average 5.2x speedup over the multi-threaded implementation of the most widely used, and optimized, open library. With a state-of-the-art CPU, we reach performance that rivals top-performing GPUs.

==> algorithm/alg-trans-share-symmetry.tex <==

\begin{algorithm}[t]
\footnotesize
\caption{Scratchpad algorithm.}
\LinesNumbered
\Input{img[nb][nw][nh], mat[nb][3][4], volume[nx][ny][nz], vecIJ}
\Output{volume[nx][ny][nz]}

{\color{blue}\#pragma omp parallel for}

\ForEach {\{i, j\} $\in$ vecIJ}{

    vec $\gets$ \{i, j, 0, 1.f\}

    \For{$s=0$ to $nb-1$}{
        F[s]{$\gets$}1.f/dot4(mat[s][2], vec)
        
        W[s]{$\gets$}F[s]*F[s]
        
        X[s]{$\gets$}dot4(mat[s][0], vec)*F[s]
    }
    

}



\end{algorithm}











==> algorithm/alg-use-sub-line.tex <==
\begin{figure}
  \centering
  \begin{minipage}{1.04\linewidth}
    \begin{algorithm}[H]
    \label{alg:scratchpad-subline}
      \footnotesize
\caption{Second interpolation by sub-line algorithm.}
\LinesNumbered
\Input{sMem, mat[nb][3][4], volume[nx][ny][nz], vecIJ\Comment{the pairs of i and j are stored in vecIJ}}
\Output{volume[nx][ny][nz]}

{\color{blue}\#pragma omp parallel for} \Comment{launch multiple threads}

\ForEach {\{i, j\} $\in$ vecIJ}{

   
    }

}
    \end{algorithm}
  \end{minipage}
\end{figure}

==> algorithm/filtering.tex <==
\begin{algorithm}[t]
\caption{Filtering computation. height$\times$width and nProj are the size and number of projections, respectively.}
\label{alg:filtering}
\LinesNumbered
\KwIn{I[nProj][height][width], $W_{cos}$, $W_{ramp}$}
\KwOut{I[nProj][height][width]}
%some description\; %\;用於換行
\For{$i = 0$ to $nProj-1$}{
    {I[i] $\gets$ Img[i] $\cdot$ $W_{cos}$} \Comment{point-wise multiplication}
}
\For {$j = 0$ to $height-1$}{
    {I[i][j] $\gets$ {I[i][j]}{$\otimes$}$W_{ramp}$} \Comment{${\otimes}$ indicates convolution}
}
\end{algorithm}

==> listings/alg-bp-batch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\rmfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by reorganizing loops and using scratchpad memory. The arguments are same to Listing~\ref{alg:bp-transpose}.}, label = alg:bp-batch]
void <@\bf{bpScratchpad\_mt}@>(......)
{
   #pragma omp parallel for
   for (int i = 0; i < nx; i++){
      for (int j = 0; j < ny; j++){
	       <@\hllightgray{float F[nb], W[nb], X[nb];}@>
	       float vec[4] = {i,j,0,1.f};
	       for (int s=0; s<nb; s++){
	          F[s] = 1.f/<@\bf{dot4}@>(mat[s][2], vec);//dot 
	          W[s] = F[s]*F[s];
	          X[s] = <@\bf{dot4}@>(mat[s][0], vec)*f;  //dot
	       }
	       for (int k = 0; k < <@{nz/2}@>; k++){
	          vec[3] = k; //update k
	          float sum=0, _sum=0;
	          float y;
	          <@\hllightgray{for (int s=0; s<nb; s++)}@>{
	             y = <@\bf{dot4}@>(mat[s][1], vec)*f;//dot
	             float val = <@\bf{subPiexl}@>(img[s], y, <@\hllightgray{X[s]}@>);
	             sum += val*<@\hllightgray{W[s]}@>;//accumulate
	             //geometry symmetry 
	             y = height - 1.f - y;
			       val = <@\bf{subPiexl}@>(img[s], y, <@\hllightgray{X[s]}@>);
			       _sum += val*<@\hllightgray{W[s]}@>;//accumulate 
	           }//s
	           volume<@{[i][j][k]}@>      += sum; //update
	           volume<[i][j][nz-1-k]  += _sum;//update 
   }   }   } // i, j, k
}
\end{lstlisting}
\end{minipage}
\end{figure}

%This is normal text.
%<@\bf\textcolor{red}{red text}@>
%More.
%%%%%%%%%%%%%%%%%%%%%%%%%

==> listings/alg-bp-ocl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}


\begin{comment}
\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by transposing projections and volume data.}, label = alg:bp-transpose]
void <@\bf{bpTransShareSymmetry}@>(const float img[nProj]<@\hllightgray{[width][height]}@>, const float mat[nProj][3][4], float volume<@\hllightgray{[nx][ny][nz]}@>)
{
	for (int s = 0; s < nProj; s++){
	   #pragma omp parallel for
	   for (int i = 0; i < nx; i++){
	      for (int j = 0; j < ny; j++){
	         float vec[4] = {i,j,0,1.f};   //coordinate(i,j,0) 
	         float z = <@\bf{dot4}@>(mat[s][2], vec);    //inner product
		      float f = 1.f/z;
		      float weight = f*f;              //compute weight
		      float x = <@\bf{dot4}@>(mat[s][0], vec)*f;  //inner product
	         for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
	            vec[3] = k;
				   float y = <@\bf{dot4}@>(mat[s][1], vec)*f;  //inner product
				   float pixel = <@\bf{subPiexl}@>(img, <@\hllightgray{y, x}@>);  //sub-pixel
				   volume<@\hllightgray{[i][j][k]}@> += pixel*weight;  //update
				   //geometry symmetry
				   y = height - 1.f - y;
				   pixel = <@\bf{subPiexl}@>(img, <@\hllightgray{y, x}@>);  //sub-pixel
				   volume<@\hllightgray{[i][j][nz-1-k]}@> += pixel*weight;  //update 
		      } //z
	      }	//j
	   } //j
	} //s
}
\end{lstlisting}
\end{minipage}
\end{figure}

\end{comment}

%This is normal text.
%<@\bf\textcolor{red}{red text}@>
%More.
%%%%%%%%%%%%%%%%%%%%%%%%%

==> listings/alg-bp-share-symmetry.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\rmfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection using geometry symmetry. The arguments are same to Listing~\ref{alg:bp-transpose}.}, label = alg:bp-trans-share-symmetry]
void <@\bf{bpSymmetry\_mt}@>(......){
	//<@\color{red}\bf{codes \& loops for s, i, j are same to line 2$\sim$8 of Lising~\ref{alg:bp-trans-share}}@>
	...... ...... ......//<@\color{red}\bf{Note: including lines 4$\sim$8 of Listing~\ref{alg:bp-trans-share}}@>
	         for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
	            vec[3] = k; //update k
				   float y = <@\bf{dot4}@>(mat[s][1], vec)*f;  //dot
				   float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				   volume<@{[i][j][k]}@> += val*weight;//update
				   //geometry symmetry
				   <@\hllightgray{y}@> = height - 1.f - y;
				   val = <@\bf{subPiexl}@>(img[s], <@{\_y, x}@>);
				   volume[i][j][<@\hllightgray{nz-1-k}@>]+=val*weight;//update 
    } }  }  } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}

==> listings/alg-bp-trans-share-symmetry.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\rmfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 2, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}



\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection using our optimizing techniques: transposing projections \& volume data, reordering loops, reusing variables after hoisting, and exploiting geometric symmetry.}, label = alg:bp-transpose]
void <@\bf{bpTransShareSymmetry}@>(float img[nb]<@\hllightgray{[nw][nh]}@>, 
    float mat[nb][3][4], float volume<@\hllightgray{[nx][ny][nz]}@>)
{
  for (int s = 0; s < nb; s++){//a batch of projections
    #pragma omp parallel for collapse(2)
    for (int i = 0; i < nx; i++){
      for (int j = 0; j < ny; j++){
        float vec[4] = {i,j,0,1.f};//coordinate
        float <@\hllightgray{z}@> = <@\bf{dot4}@>(mat[s][2], vec);//dot
	      float <@\hllightgray{f}@> = 1.f/z;
	      float <@\hllightgray{w}@> = f*f;  //compute weight
	      float <@\hllightgray{x}@> = <@\bf{dot4}@>(mat[s][0], vec)*f;//dot
        for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
           vec[3] = k; //update k
	         float y = <@\bf{dot4}@>(mat[s][1], vec)*f; //dot
	         float val = <@\bf{Bilinear\_Inpterpolate}@>(img[s], <@{y, x}@>);
	         volume[i][j][k] += val*w;//update
	         float <@\hllightgray{\_y}@> = height-1.f-y;//geometry symmetry
	         val = <@\bf{Bilinear\_Inpterpolate}@>(img[s], _y, x);
	         int <@\hllightgray{\_k}@> = nz-1-k;//index symmetry
	         volume[i][j][_k] += val*w;//update 
  } } } } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}


\begin{comment}
\begin{figure}[t]
  \begin{minipage}{.485\textwidth}
    \centering
    \lstset{numbers=left,xleftmargin=2em,breaklines,language=C++, aboveskip=0pt,belowskip=0pt}
    \lstinputlisting[lastline=1]{bp.cpp}
    \lstinputlisting[backgroundcolor=\color{orange!30},firstline=2,lastline=2, firstnumber=2]{bp.cpp}
    \lstinputlisting[firstline=3, firstnumber=3]{bp.cpp}
  \end{minipage}
\end{figure}








\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by our optimizing techniques: transposing projections & volume data, share variables, and geometric symmetry.}, label = alg:bp-transpose]
void <@\bf{bpTransShareSymmetry\_mt}@>(float img[nb]<@\hllightgray{[nw][nh]}@>, 
    float mat[nb][3][4], float volume<@\hllightgray{[nx][ny][nz]}@>)
{
  for (int s = 0; s < nb; s++){
    #pragma omp parallel for
    for (int i = 0; i < nx; i++){
      for (int j = 0; j < ny; j++){
        float vec[4] = {i,j,0,1.f};//coordinate
        float <@\hllightgray{z}@> = <@\bf{dot4}@>(mat[s][2], vec);//dot
	      float <@\hllightgray{f}@> = 1.f/z;
	      float <@\hllightgray{weight}@> = f*f;  //compute weight
	      float <@\hllightgray{x}@> = <@\bf{dot4}@>(mat[s][0], vec)*f;//dot
        for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
           vec[3] = k; //update k
	         float y = <@\bf{dot4}@>(mat[s][1], vec)*f; //dot
	         float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
	         volume[i][j][k] += val*weight;//update
	         float <@\hllightgray{\_y}@> = height-1.f-y;//geometry symmetry
	         val = <@\bf{subPiexl}@>(img[s], _y, x);
	         int <@\hllightgray{\_k}@> = nz-1-k;//index symmetry
	         volume[i][j][_k] += val*weight;//update 
  } } } } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}


\end{comment}

\begin{comment}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection using sharing variable and geometry symmetry techniques. The arguments and loop (i.e. for s, i, j) are same to Listing~\ref{alg:bp-transpose}.}, label = alg:bp-trans-share-symmetry]
void <@\bf{bpShareSymmetry\_mt}@>(......){
	      float vec[4] = {i,j,0,1.f};//coordinate
	      float <@\hllightgray{z}@> = <@\bf{dot4}@>(mat[s][2], vec);//dot
		   float <@\hllightgray{f}@> = 1.f/z;
		   float <@\hllightgray{weight}@> = f*f;  //compute weight
		   float <@\hllightgray{x}@> = <@\bf{dot4}@>(mat[s][0], vec)*f;//dot
	      for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
	         vec[3] = k; //update k
				float y = <@\bf{dot4}@>(mat[s][1], vec)*f; //dot
				float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				volume<@{[i][j][k]}@> += val*weight;//update
				float <@\hllightgray{\_y}@> = height-1.f-y;//geometry symmetry
				val = <@\bf{subPiexl}@>(img[s], _y, x);
				int <@\hllightgray{\_k}@> = nz-1-k;//index symmetry
				volume[i][j][_k]+=val*weight;//update 
   } } } } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}

%This is normal text.
%<@\bf\textcolor{red}{red text}@>
%More.
%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection using geometry symmetry. The arguments are same to Listing~\ref{alg:bp-transpose}.}, label = alg:bp-trans-share-symmetry]
void <@\bf{bpSymmetry\_mt}@>(......){
	//<@\color{red}\bf{codes \& loops for s, i, j are same to line 2$\sim$8 of Lising~\ref{alg:bp-trans-share}}@>
	...... ...... ......//<@\color{red}\bf{Note: including lines 4$\sim$8 of Listing~\ref{alg:bp-trans-share}}@>
	         for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
	            vec[3] = k; //update k
				   float y = <@\bf{dot4}@>(mat[s][1], vec)*f;  //dot
				   float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				   volume<@{[i][j][k]}@> += val*weight;//update
				   //geometry symmetry
				   <@\hllightgray{y}@> = height - 1.f - y;
				   val = <@\bf{subPiexl}@>(img[s], <@{\_y, x}@>);
				   volume[i][j][<@\hllightgray{nz-1-k}@>]+=val*weight;//update 
    } }  }  } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}



\begin{figure}[t!]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by transposing projections and volume data.}, label = alg:bp-trans-share-symmetry]
void <@\bf{bpSymmetry}@>(float img[nProj]<@{[width][height]}@>, float mat[nProj][3][4], float volume<@{[nx][ny][nz]}@>)
{
	for (int s = 0; s < nProj; s++){
	   #pragma omp parallel for
	   for (int i = 0; i < nx; i++){
	      for (int j = 0; j < ny; j++){
	         float vec[4] = {i,j,0,1.f};//coordinate(i,j,0) 
	         float z = <@\bf{dot4}@>(mat[s][2], vec);    //dot
		      float f = 1.f/z;
		      float weight = f*f;              //compute weight
		      float x = <@\bf{dot4}@>(mat[s][0], vec)*f;  //dot
	         for (int k = 0; k < <@\hllightgray{nz/2}@>; k++){
	            vec[3] = k; //update k
				   float y = <@\bf{dot4}@>(mat[s][1], vec)*f;  //dot
				   float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				   volume<@{[i][j][k]}@> += val*weight;//update
				   //geometry symmetry
				   <@\hllightgray{y}@> = height - 1.f - y;
				   val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				   volume[i][j][<@\hllightgray{nz-1-k}@>] += val*weight;//update 
    } }  }  } // s, i, j ,k
}
\end{lstlisting}
\end{minipage}
\end{figure}
\end{comment}

==> listings/alg-bp-transpose-sharedata.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\rmfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}


\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by sharing variables. The arguments are same to Listing~\ref{alg:bp-transpose}.}, label = alg:bp-trans-share]
void <@\bf{bpShare\_mt}@>(......){
    //<@\color{red}\bf{codes \& loops for s, i, j are same to line 3$\sim$6 of Lising~\ref{alg:bp-transpose}}@>
    ......   ......   ......   ......   ......
	          float vec[4] = {i,j,0,1.f};//coordinate
	          float <@\hllightgray{z}@> = <@\bf{dot4}@>(mat[s][2], vec);//dot
		       float <@\hllightgray{f}@> = 1.f/z;
		       float <@\hllightgray{weight}@> = f*f;  //compute weight
		       float <@\hllightgray{x}@> = <@\bf{dot4}@>(mat[s][0], vec)*f;//dot
	          for (int k = 0; k < nz; k++){
	              vec[3] = k;//update k
				     float y = <@\bf{dot4}@>(mat[s][1], vec)*f;//dot
				     float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				     volume<@{[i][j][k]}@> += val*weight;  //update 
    } }  }  } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}

%This is normal text.
%<@\bf\textcolor{red}{red text}@>
%More.
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[t!]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by transposing projections and volume data.}, label = alg:bp-trans-share]
void <@\bf{bpShare}@>(float img[nProj]<@{[width][height]}@>, float mat[nProj][3][4], float volume<@{[nx][ny][nz]}@>)
{
	for (int s = 0; s < nProj; s++){
	   #pragma omp parallel for
	   for (int i = 0; i < nx; i++){
	      for (int j = 0; j < ny; j++){
	          float vec[4] = {i,j,0,1.f};//coordinate
	          float <@\hllightgray{z}@> = <@\bf{dot4}@>(mat[s][2], vec);//dot
		       float <@\hllightgray{f}@> = 1.f/z;
		       float <@\hllightgray{weight}@> = f*f;  //compute weight
		       float <@\hllightgray{x}@> = <@\bf{dot4}@>(mat[s][0], vec)*f;//dot
	          for (int k = 0; k < nz; k++){
	              vec[3] = k; //update k
				     float y = <@\bf{dot4}@>(mat[s][1], vec)*f;  //dot
				     float val = <@\bf{subPiexl}@>(img[s], <@{y, x}@>);
				     volume<@{[i][j][k]}@> += val*weight;  //update 
    } } } } // s, k, j ,i
}
\end{lstlisting}
\end{minipage}
\end{figure}
\end{comment}

==> listings/alg-bp-transpose.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\rmfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 3, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.49\textwidth}
\begin{lstlisting}[caption = {The proposed back-projection by transposing projections and volume data.}, label = alg:bp-transpose]
void <@\bf{bpTranspose\_mt}@>(float img[nProj]<@\hllightgray{[width][height]}@>, 
    float mat[nProj][3][4], float volume<@\hllightgray{[nx][ny][nz]}@>)
{
	for (int s = 0; s < nProj; s++){
	   #pragma omp parallel for
	   for (int i = 0; i < nx; i++){
	      for (int j = 0; j < ny; j++){
	         <@\hllightgray{for (int k = 0; k < nz; k++)}@>{
	            float vec[4] = {i,j,k,1.f};//coordinate
				   float z = <@\bf{dot4}@>(mat[s][2], vec);//dot
				   float f = 1.f/z;
				   float x = <@\bf{dot4}@>(mat[s][0], vec)*f; //dot
				   float y = <@\bf{dot4}@>(mat[s][1], vec)*f; //dot
				   float val = <@\bf{subPiexl}@>(img[s], <@\hllightgray{y, x}@>);
				   float weight = f*f;//compute weight
				   volume<@\hllightgray{[i][j][k]}@> += val*weight;//update
    }  }  }  } // k, j, i, s
}
\end{lstlisting}
\end{minipage}
\end{figure}

%This is normal text.
%<@\bf\textcolor{red}{red text}@>
%More.
%%%%%%%%%%%%%%%%%%%%%%%%%
%		      } //i
%	      }	//j
%	   } //k
%	} //s

==> listings/alg-subpixel.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
 	language = C++, breaklines = true, breakindent = 10pt, basicstyle = \rmfamily\scriptsize, commentstyle = {\itshape \color[cmyk]{1,0.4,1,0}}, classoffset = 0, keywordstyle = {\bfseries \color[cmyk]{0,1,0,0}}, stringstyle = {\ttfamily \color[rgb]{0,0,1}}, frame = trbl, framesep=5pt, numbers = left, stepnumber = 1, xrightmargin=7pt, xleftmargin=8pt, numberstyle = \tiny, tabsize = 2, captionpos = t, directivestyle={\color{black}},  emph={int,char,double,float,unsigned}, emphstyle={\color{blue}},
}
\lstset{escapeinside={<@}{@>}}

\begin{figure}[t]
\centering
\begin{minipage}[c]{0.5\textwidth}
\begin{lstlisting}[caption = {Proposed scheme for bi-linear interpolation.}, label = alg:subpixel]
float <@\bf{subPiexl}@>(float img[nh][nw], float x, float y)
{
  int nx = (int)x; //convert to integer
  int ny = (int)y; //convert to integer
	//horizontal interpolation using mix function
	float s0 = <@\bf{mix}@>(img[ny  ][nx], img[ny  ][nx+1], x-nx);
	float s1 = <@\bf{mix}@>(img[ny+1][nx], img[ny+1][nx+1], x-nx);
	//vertical interpolation using mix function
	return mix(s0, s1, y-ny);
}
\end{lstlisting}
\end{minipage}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%

==> macro.tex <==
\newcommand{\tbhline}{\noalign{\hrule height 1pt}}
\newcommand\inner[2]{\langle #1, #2 \rangle}

\newcolumntype{|}{!{\vrule width 0.5pt}}
\newcolumntype{?}{!{\vrule width 1pt}}
\newcolumntype{^}{!{\vrule width 1.2pt}}


\renewcommand{\O}[1]{$\mathcal{O}(#1)$}


\newcommand{\bhline}[1]{\noalign{\hrule height #1}}    
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}    

%\renewcommand{\theenumi}{\ajMaru{enumi}}


% remove end sentences
\algtext*{EndWhile}
\algtext*{EndIf}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\Break}{\textbf{break}}

\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\newcommand{\twoKperf}{20}
\newcommand{\fourKperf}{30}
\newcommand{\eightKperf}{2}

\newcommand{\iFDK}{\ding{iFDK}}%


% Nice little colorful numbered boxes
\definecolor{myblue}{RGB}{91,155,213}
\definecolor{mydark}{RGB}{0,0,0}
\newcommand*\circled[1]{\color{white}\tikz[baseline=(char.base)]{
		\node[shape=circle,inner sep=0.5pt,fill=myblue] (char) {#1};}\color{black}\,}
\newcommand*\circledempty[1]{\color{black}\tikz[baseline=(char.base)]{
		\node[shape=circle, draw=myblue, thin, inner sep=0.5pt,fill=white] (char) {#1};}\color{black}\,}
		
		
		
\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{cyan}\hl{#1}}}
\DeclareRobustCommand{\hllightgray}[1]{{\sethlcolor{lightgray}\hl{#1}}}
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}


\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output\,}
\SetKwInOut{Data}{Data}
\SetKwProg{Tree}{Tree}{}{EndTree}


\newcommand{\rOne}{\ding{\rotatebox{90}{$256^2\times512\rightarrow256^3$}}}%
\newcommand{\rTwo}{\ding{\rotatebox{90}{$256^2\times512\rightarrow512^3$}}}%
\newcommand{\rThree}{\ding{\rotatebox{90}{$256^2\times512\rightarrow1024^3$}}}%
\newcommand{\rFour}{\ding{\rotatebox{90}{$512^2\times512\rightarrow256^3$}}}%
\newcommand{\rFive}{\ding{\rotatebox{90}{$512^2\times512\rightarrow512^3$}}}%
\newcommand{\rSix}{\ding{\rotatebox{90}{$512^2\times512\rightarrow1024^3$}}}%
\newcommand{\rSeven}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow256^3$}}}%
\newcommand{\rEight}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow512^3$}}}%
\newcommand{\rNine}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow1024^3$}}}%


\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}

==> tables/tbl-scaling.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}[t]  
      \caption{Scaling the Performance of the Baseline Implementation~\cite{rit2014reconstruction} (see Listing~\ref{alg:bp-baseline}). The Number of physical cores is in Table~\ref{tbl:evaluation-env}}        
      %\small
      \centering
      \resizebox{\linewidth}{!}{
      \begin{tabular}{ ?c|c|c|c|c|c|c|c? }
      \tbhline
      \bf{Threads}     & 1    & 2    & 4    & 8    & 16   & 32   & 64   \\
      \tbhline
      E5-2630\_v4      & 0.07 & 0.13 & 0.26 & 0.52 & 1.04 & 1.21 & 1.32  \\
      E5-2650\_v3      & 0.06 & 0.12 & 0.26 & 0.51 & 1.02 & 1.24 & 1.34  \\
      Gold\_6140       & 0.11 & 0.22 & 0.42 & 0.81 & 1.59 & 2.88 & 2.69 \\
      i7-9700K         & 0.16 & 0.31 & 0.60 & 1.13 & 1.07 &  -   & -    \\
      \tbhline
      \end{tabular}  }
      \label{tbl:evaluation-env} 
\end{table}     
%%%%%%%%%%%%%%%%%%%%%%%%%





\begin{comment}
      \multirow{2}{*}{\bf{Intel CPU}}  & \bf{Xeon}    & \bf{Xeon}  &\bf{Xeon}  & \bf{Core}\\
       \bf{}  & \bf{E5-2630 v4}    & \bf{E5-2650 v3}  &\bf{Gold 6140}  & \bf{i7-9700K}\\
          Cores           &      10         & 10               &18              & 8 \\
          Threads/core    &      2          & 2                & 1              &1\\
          Frequency       &   {2.2GHz}    & {2.3GHz}       &{2.3GHz}      & {3.6GHz}\\  
          Sockets         &   {2}         & {2}            &{2}           & {1}\\
          GFLOPS          &   {704}         & {736}            &{2,650}           & {461}\\
          Max bandwidth          &   {137 GB/s}         & {137 GB/s}        &{250  GB/s}      & {42  GB/s}\\
%         CPU Stream Rates        &   {-}         & {-}        &{-}      & {-}\\
      \hline
          Memory          &    256GB        & 256GB            &192GB           & 32GB        \\       
     \hline
          OS              & CentOS 7.4      & CentOS 7.4       & CentOS 7.4     & Ubuntu 16.04\\

\begin{table}[]
\begin{tabular}{llllllll}
            & 1    & 2    & 4    & 8    & 16   & 32   & 64   \\
E5-2630\_v4 & 0.07 & 0.13 & 0.26 & 0.52 & 1.04 & 1.21 & 1.32 \\
E5-2650\_v3 & 0.06 & 0.12 & 0.26 & 0.51 & 1.02 & 1.24 & 1.34 \\
Gold\_6140  & 0.11 & 0.22 & 0.42 & 0.81 & 1.59 & 2.88 & 2.69 \\
i7-9700K    & 0.16 & 0.31 & 0.60 & 1.13 & 1.07 &      &     
\end{tabular}
\end{table}

\end{comment}

==> tables/tbl_compiler_option.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}[t]  
      \caption{Evaluation Environment}        
      \scriptsize
      \centering
      \resizebox{\linewidth}{!}{
      \begin{tabular}{ |c|c| }
      %              warsaw             rwbc-v100        personal
      \tbhline
       \bf{Compiler}  & \bf{Options}        \\
          g++           &      -fopenmp -lpthread -std=c++11         \\
      \hline
          ioc           &    -cl-mad-enable -cl-fast-relaxed-math    \\  
      \tbhline
      \end{tabular}  }
      \label{tbl:compiler-option} 
\end{table}     
%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/tbl_performance.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}[t]  
      \caption{Performance of Back-projection on CPUs Using OpenMP and OpenCL in (Batch Number is Fixed as 32)}
      %\normalsize
      %\scriptsize
      \small
      \centering
      \resizebox{\linewidth}{!}{
      \begin{tabular}{ ?c|l?c|c|c|c|c|c|c|c|c? }
      \tbhline
      \multirow{2}{*}{\rotatebox{90}{CPU}}             &\multirow{2}{*}{\bf{kernel}} & \multicolumn{9}{c?}{\bf{Performance (GUPS)}}                  \\  \cline{3-11}
                                            &                             & P1 & P2 & P3 & P4 & P5 & P6 & P7 & P8 & P9                    \\ 
      
      \tbhline
      \multirow{5}{*}{\rotatebox{90}{E5-2630$\times$2}} & baseline       & 1.22 & 1.27 & 1.35 & 1.25 & 1.29 & 1.37 & 1.12 & 1.28 & 1.37  \\  
                                                        & transpose\_mp  & 1.05 & 1.23 & 1.32 & 1.04 & 1.24 & 1.32 & 1.03 & 1.27 & 1.33 \\
                                                        & share\_mp      & 1.45 & 1.63 & 1.75 & 1.41 & 1.59 & 1.74 & 1.21 & 1.64 & 1.77 \\
                                                        & symmetry\_mp   & 1.52 & 1.67 & 1.84 & 1.50 & 1.71 & 1.84 & 1.48 & 1.68 & 1.86 \\
                                                        & scratchpad\_mp & 1.30 & 1.43 & 1.54 & 1.36 & 1.50 & 1.53 & 0.89 & 1.10 & 1.25 \\
     \cline{1-11}
     \multirow{5}{*}{\rotatebox{90}{E5-2650$\times$2}} & baseline   & 1.25 & 1.30 & 1.38 & 1.29 & 1.30 & 1.41 & 1.22 & 1.31 & 1.41   \\  
                                        & transpose\_mp  & 1.08 & 1.27 & 1.36 & 1.08 & 1.27 & 1.36 & 1.04 & 1.28 & 1.36  \\
                                        & share\_mp      & 1.43 & 1.67 & 1.81 & 1.42 & 1.68 & 1.81 & 1.35 & 1.66 & 1.81 \\
                                        & symmetry\_mp   & 1.54 & 1.73 & 1.91 & 1.55 & 1.78 & 1.91 & 1.53 & 1.75 & 1.93 \\
                                        & scratchpad\_mp      & 1.46 & 1.56 & 1.61 & 1.43 & 1.56 & 1.61 & 0.92 & 1.12 & 1.30 \\
     \cline{1-11}
     \multirow{5}{*}{\rotatebox{90}{Gold-6140$\times$2}} & baseline   & 2.52 & 2.65 & 2.63 & 2.52 & 2.64 & 2.78 & 2.31 & 2.58 & 2.72 \\  
                                        & transpose\_mp  & 2.43 & 2.59 & 2.64 & 2.38 & 2.53 & 2.69 & 2.28 & 2.53 & 2.65 \\
                                        & share\_mp      & 3.18 & 3.44 & 3.49 & 3.14 & 3.46 & 3.58 & 2.91 & 3.40 & 3.50 \\
                                        & symmetry\_mp   & 3.41 & 3.29 & 3.40 & 3.20 & 3.41 & 3.37 & 3.02 & 3.49 & 3.55 \\
                                        & scratchpad\_mp      & 2.19 & 2.81 & 2.85 & 1.71 & 2.80 & 2.96 & 1.67 & 1.99 & 2.92 \\  
     \cline{1-11}
     \multirow{5}{*}{\rotatebox{90}{i7-9700K$\times$1}} & baseline   & 0.95 & 0.95 & 0.93 & 0.91 & 0.93 & 0.93 & 0.88 & 0.92 & 0.92  \\  
                                        & transpose\_mp  & 0.91 & 0.92 & 0.91 & 0.89 & 0.90 & 0.91 & 0.89 & 0.90 & 0.90  \\
                                        & share\_mp      & 1.29 & 1.30 & 1.30 & 1.27 & 1.28 & 1.29 & 1.25 & 1.27 & 1.29 \\
                                        & symmetry\_mp   & 1.31 & 1.20 & 1.18 & 1.31 & 1.22 & 1.19 & 1.29 & 1.28 & 1.24  \\
                                        & scratchpad\_mp      & 0.91 & 0.93 & 0.92 & 0.88 & 0.93 & 0.96 & 0.65 & 0.80 & 0.86 \\                                                 
     \tbhline
     \end{tabular}  }
     \label{tbl:performance} 
\end{table*}     
%%%%%%%%%%%%%%%%%%%%%%%%%




\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}[t]  
      \caption{Performance of back-projection on CPUs by OpenMP and OpenCL in an unit of GUPS. The batch number is fixed as 32.}
      %\normalsize
      %\scriptsize
      \tiny
      \centering
      \begin{tabular}{ ?c|c|l?c|c|c|c|c|c|c|c|c? }
      \tbhline
      & \multirow{2}{*}{\bf{CPU}}             &\multirow{2}{*}{\bf{kernel}} & \multicolumn{9}{c?}{\bf{Performance (GUPS)}}                  \\  \cline{4-12}
      &                                       &                             & P1 & P2 & P3 & P4 & P5 & P6 & P7 & P8 & P9  \\ 
      
      \tbhline
   \multirow{20}{*}{\rotatebox{90}{OpenMP}}   &\multirow{5}{*}{\rotatebox{90}{E5-2630$\times$2}} & baseline       & 1.22 & 1.27 & 1.35 & 1.25 & 1.29 & 1.37 & 1.12 & 1.28 & 1.37  \\  
      &                                  & transpose\_mp  & 1.05 & 1.23 & 1.32 & 1.04 & 1.24 & 1.32 & 1.03 & 1.27 & 1.33 \\
      &                                  & share\_mp      & 1.45 & 1.63 & 1.75 & 1.41 & 1.59 & 1.74 & 1.21 & 1.64 & 1.77 \\
      &                                  & symmetry\_mp   & 1.52 & 1.67 & 1.84 & 1.50 & 1.71 & 1.84 & 1.48 & 1.68 & 1.86 \\
      &                                  & scratchpad\_mp & 1.30 & 1.43 & 1.54 & 1.36 & 1.50 & 1.53 & 0.89 & 1.10 & 1.25 \\
      \cline{2-12}
      & \multirow{5}{*}{\rotatebox{90}{E5-2650$\times$2}} & baseline   & 1.25 & 1.30 & 1.38 & 1.29 & 1.30 & 1.41 & 1.22 & 1.31 & 1.41   \\  
      &                                  & transpose\_mp  & 1.08 & 1.27 & 1.36 & 1.08 & 1.27 & 1.36 & 1.04 & 1.28 & 1.36  \\
      &                                  & share\_mp      & 1.43 & 1.67 & 1.81 & 1.42 & 1.68 & 1.81 & 1.35 & 1.66 & 1.81 \\
      &                                  & symmetry\_mp   & 1.54 & 1.73 & 1.91 & 1.55 & 1.78 & 1.91 & 1.53 & 1.75 & 1.93 \\
      &                                  & scratchpad\_mp      & 1.46 & 1.56 & 1.61 & 1.43 & 1.56 & 1.61 & 0.92 & 1.12 & 1.30 \\
      \cline{2-12}
      &\multirow{5}{*}{\rotatebox{90}{Gold-6140$\times$2}} & baseline   & 2.52 & 2.65 & 2.63 & 2.52 & 2.64 & 2.78 & 2.31 & 2.58 & 2.72 \\  
      &                                  & transpose\_mp  & 2.43 & 2.59 & 2.64 & 2.38 & 2.53 & 2.69 & 2.28 & 2.53 & 2.65 \\
      &                                  & share\_mp      & 3.18 & 3.44 & 3.49 & 3.14 & 3.46 & 3.58 & 2.91 & 3.40 & 3.50 \\
      &                                  & symmetry\_mp   & 3.41 & 3.29 & 3.40 & 3.20 & 3.41 & 3.37 & 3.02 & 3.49 & 3.55 \\
      &                                  & scratchpad\_mp      & 2.19 & 2.81 & 2.85 & 1.71 & 2.80 & 2.96 & 1.67 & 1.99 & 2.92 \\  
      \cline{2-12}
      &\multirow{5}{*}{\rotatebox{90}{i7-9700K$\times$1}} & baseline   & 0.95 & 0.95 & 0.93 & 0.91 & 0.93 & 0.93 & 0.88 & 0.92 & 0.92  \\  
      &                                  & transpose\_mp  & 0.91 & 0.92 & 0.91 & 0.89 & 0.90 & 0.91 & 0.89 & 0.90 & 0.90  \\
      &                                  & share\_mp      & 1.29 & 1.30 & 1.30 & 1.27 & 1.28 & 1.29 & 1.25 & 1.27 & 1.29 \\
      &                                  & symmetry\_mp   & 1.31 & 1.20 & 1.18 & 1.31 & 1.22 & 1.19 & 1.29 & 1.28 & 1.24  \\
      &                                  & scratchpad\_mp      & 0.91 & 0.93 & 0.92 & 0.88 & 0.93 & 0.96 & 0.65 & 0.80 & 0.86 \\         
      \tbhline
      \multirow{24}{*}{\rotatebox{90}{OpenCL}} &\multirow{6}{*}{\rotatebox{90}{E5-2630$\times$2}}  &  transpose\_cl        & 3.10 & 3.28 & 3.30 & 2.87 & 3.17 & 3.21 & 1.53 & 2.55 & 2.76  \\
      &                                                   &  share\_cl           & 5.09 & 5.58 & 5.70 & 4.58 & 5.33 & 5.53 & 2.02 & 3.82 & 4.64 \\
      &                                                   &  share\_lm\_cl       & 6.23 & 7.58 & 7.84 & 5.06 & 6.69 & 7.27 & 2.75 & 4.42 & 6.37 \\
      &                                                   &  symmetry\_cl        & 4.97 & 5.51 & 5.59 & 4.24 & 4.99 & 5.19 & 1.91 & 3.11 & 4.11 \\
      &                                                   &  symmetry\_lm\_cl    & 7.82 & 9.56 & 10.2 & 6.37 & 8.30 & 9.40 & 3.18 & 5.56 & 7.58 \\
      &                                                   &  symmetry\_pf\_cl    & \color{blue}8.10 & \color{blue}9.78 & \color{blue}10.8 & \color{blue}6.40 & \color{blue}8.58 & \color{blue}9.93 & \color{blue}3.15 & \color{blue}5.75 & \color{blue}8.08 \\
      \cline{2-12}
      &\multirow{6}{*}{\rotatebox{90}{E5-2650$\times$2}}  &  transpose\_cl        & 3.23 & 3.40 & 3.43 & 3.03 & 3.30 & 3.33 & 1.49 & 2.61 & 2.84  \\
      &                                                   &  share\_cl           & 5.34 & 5.86 & 5.94 & 4.92 & 5.64 & 5.79 & 1.88 & 3.81 & 4.72  \\
      &                                                   &  share\_lm\_cl       & 6.53 & 7.85 & 8.18 & 5.34 & 7.02 & 7.66 & 2.26 & 4.40 & 6.64  \\
      &                                                   &  symmetry\_cl        & 5.15 & 5.64 & 5.69 & 4.48 & 5.17 & 5.25 & 1.84 & 3.19 & 4.22  \\
      &                                                   &  symmetry\_lm\_cl    & 8.23 & 10.0 & 10.8 & 6.74 & 8.83 & 9.90 & 2.48 & 5.36 & 7.97  \\
      &                                                   &  symmetry\_pf\_cl    & \color{blue}8.52 & \color{blue}10.2 & \color{blue}11.3 & \color{blue}6.85 & \color{blue}9.11 & \color{blue}10.3 & \color{blue}2.48 & \color{blue}5.44 & \color{blue}8.48  \\
      \cline{2-12}      
      &\multirow{6}{*}{\rotatebox{90}{Gold-6140$\times$2}}&  transpose\_cl        & 5.45 & 5.94 & 6.03 & 4.70 & 5.92 & 6.06 & 2.65 & 4.05 & 5.93  \\
      &                                                   &  share\_cl           & 9.02 & 11.3 & 11.8 & 7.25 & 11.1 & 11.8 & 3.95 & 6.38 & 11.2 \\
      &                                                   &  share\_lm\_cl       & 13.1 & 17.7 & 19.4 & 10.1 & 15.6 & 17.9 & 4.94 & 10.2 & 15.4 \\
      &                                                   &  symmetry\_cl        & 9.50 & 11.9 & 12.6 & 7.18 & 11.3 & 12.4 & 3.76 & 5.90 & 10.4 \\
      &                                                   &  symmetry\_lm\_cl    & 16.4 & 24.8 & 28.8 & 11.6 & 21.4 & 26.6 & 5.52 & 11.2 & 20.4 \\
      &                                                   &  symmetry\_pf\_cl    & \color{blue}15.9 & \color{blue}25.0 & \color{blue}27.9 & \color{blue}11.3 & \color{blue}21.6 & \color{blue}26.8 & \color{blue}5.37 & \color{blue}11.1 & \color{blue}20.8 \\
      \cline{2-12}
      &\multirow{6}{*}{\rotatebox{90}{i7-9700K$\times$1}} &  transpose\_cl        & 2.00 & 1.92 & 1.91 & 1.87 & 1.88 & 1.90 & 1.06 & 1.58 & 1.72 \\
      &                                                   &  share\_cl           & 3.05 & 3.14 & 2.93 & 2.76 & 3.14 & 2.98 & 1.19 & 2.28 & 2.58 \\
      &                                                   &  share\_lm\_cl       & 4.70 & 5.37 & 5.49 & 2.88 & 4.62 & 4.97 & 1.04 & 2.41 & 4.25 \\
      &                                                   &  symmetry\_cl        & 3.51 & 3.63 & 3.34 & 2.54 & 3.22 & 3.16 & 1.12 & 1.97 & 2.54 \\
      &                                                   &  symmetry\_lm\_cl    & 5.63 & 6.34 & 6.36 & 3.34 & 5.03 & 5.89 & 1.14 & 2.57 & 4.58 \\
      &                                                   &  symmetry\_pf\_cl    & \color{blue}6.03 & \color{blue}7.03 & \color{blue}6.99 & \color{blue}3.39 & \color{blue}5.31 & \color{blue}6.40 & \color{blue}1.15 & \color{blue}2.54 & \color{blue}4.72 \\        
       \tbhline
       \end{tabular}  
      \label{tbl:performance} 
\end{table*}     
%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}
